Equity2Vec: End-to-end Deep Learning Framework for Cross-sectional Asset Pricing

Pricing assets has attracted significant attention from the financial technology community. We observe that the existing solutions overlook the cross-sectional effects and not fully leveraged the heterogeneous data sets, leading to sub-optimal performance. To this end, we propose an end-to-end deep learning framework to price the assets. Our framework possesses two main properties: 1) We propose Equity2Vec, a graph-based component that effectively captures both long-term and evolving cross-sectional interactions. 2) The framework simultaneously leverages all the available heterogeneous alpha sources including technical indicators, financial news signals, and cross-sectional signals. Experimental results on datasets from the real-world stock market show that our approach outperforms the existing state-of-the-art approaches. Furthermore, market trading simulations demonstrate that our framework monetizes the signals effectively.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> abstract.tex <==

 
\begin{abstract}
We propose an integrated deep learning architecture for asset pricing problem . Our architecture simultaneously leverages all the available \mc{heterogeneous} alpha sources. Our pool of alphas includes technical indicators, financial news signals, and cross-sectional signals. Our architecture possesses three main properties. 
%
First, it eludes the often encountered  overfitting issues. Although we consume a large number of technical indicators, our pipeline enjoys better generalization properties compared to linear models. 
% 
Second, our model effectively captures the interactions between signals from different categories.  
%
Third,  our architecture has a low computational cost. We design a graph-based component that extracts cross-sectional interactions, which circumvents the usage of the SVD typically employed  in standard models. 
% 
Experimental results on real-world stock market data show that our approach outperforms the existing baselines. Furthermore, the results from different trading simulators demonstrate that we can effectively monetize the signals.
% \mc{even after accounting for transaction fees. (?)}  
% \qq{we did not consider the transaction fees}
\end{abstract}

%%
%% The code below is generated by the tool at http://dl.acm.org/ccs.cfm.
%% Please copy and paste the code instead of the example below.
%%


%%
%% Keywords. The author(s) should pick words that accurately describe
%% the work being presented. Separate the keywords with commas.
%\keywords{\textsc{Stock2Vec}, Financial time series, Stock price prediction, News sentiment.}
%\vspace{1mm}
%\mc{problem} \MC{shall we rephrase as for the "asset pricing problem"?


==> dump.tex <==
\begin{itemize}
    \item Deep learning models did not leverage the cross-sectional well try to use the stock graph to, first highlight the design for graph, and then say there are a lot of methods
    but what's the limitations and the challenges, and why we use news
    \item Then we say, we have the initialization
\end{itemize}



One model --> one stock
x_i^t embedding stock i
x_j^t is embedding for stock j
f(x) -> r_i^{t+1}
inner -> x_i^t^T * x_j^t
inner product is large
f(x_i, z) f(x_j, z)

corr(r_i,r_j)

f---> linear 
(x_i)
(x_j)

Ground truth:


assume r_i or r_j  


Infer model is simplier >> |(x_i,z_i), (x_j,z_j)|

model1. f(x_i,z_i) with line 17

model2. f(h_i, z_i), h_i is random > stock index 

model3. f(z_i) more flexible

model4. f_i(z_i)  simpler 

f_i(x_i, z_i), f_j(x_i, z_j) --> 

model5. adding neighbors on top of model 1

The number of neighbors vs the training -testing gap













Tempral graph based on the time t 


(1) s_i, s_j are close, and 



1.case (z_i^t, z_j^t) 
x_i^t, x_j^t 




==> intro.tex <==
\section{Introduction}
This paper examines the design of deep learning algorithms to forecast equities (stocks) return. While this research question had been asked long ago and has a rich literature behind~\cite{hu2018listening,ticknor2013bayesian,ding2015deep,goccken2016integrating,zhang2017stock,rather2015recurrent}, including works that doubted its legitimacy~\cite{de2018advances}, it became clear that machine learning is a powerful tool for asset management. Such lines of work have significantly increased in popularity in recent years, mostly fueled by the fact that a large collection of high-quality financial data sets have become available. Roughly speaking, there have been two main schools of thought building machine learning (ML) models for pricing assets: 
% 
(i) \emph{financial professionals} who treat ML tools as black boxes that can learn non-linear relationships, which they \textit{plug-in} into their existing factor research framework, and 
% 
(ii) \emph{computer scientists} who treat the task at hand as yet-another machine learning problem, and aim to generalize existing building blocks (e.g., NLP modules~\cite{xing2018natural,herz2012stock} or LSTM models \cite{akita2016deep,rather2015recurrent}) for time series arising from stock prices data. 

\smallskip 
\noindent{\textbf{Limitation of existing models.}} Perhaps surprisingly, efforts from financial professionals and computer scientists seem to be disjoint, with little work being done 
% ; minimum works were done
to address cross-cutting constraints arising across both finance and machine learning communities. We briefly discuss three major weaknesses of existing models.

\noindent{\emph{1. The source of alpha is not identified.}} Many machine learning models (especially those that rely only on news as the data source) do not examine the source of alpha (i.e., the reason why the model is able to make money). For example, a stock with recent robust return may result in media attention with positive commentary. Following that, an NLP-based model may pick up the news’ positive sentiment and predict that the stock price will continue to rise. However, this is essentially a ``momentum'' strategy \cite{bollen2011twitter,pagolu2016sentiment}, and thus the NLP-based model faces two main issues: (i) the model could be more effective if it can directly use price information, instead of news;  (ii) a momentum strategy is usually considered as ``low quality'' alpha (i.e., low return and Sharpe).

\noindent{\emph{2. Heterogeneous data sets are not used.}} Most models use only one type of data (i.e., either news text or ``factors'' \cite{ming2014stock,hu2018listening,mittermayer2006newscats,wu2019adaptive,patel2015predicting}  in numeric form). It remains open to build a model that leverages heterogeneous data and alpha sources. This model needs to reconcile (sometimes contradictory) information from different data sources. 

\noindent{\emph{3. Cross-sectional effects are not properly leveraged.}} Another salient property of the equity return forecasting problem is that the training pairs $(X, y)$ are not independent. For example, when Google has a positive return, it is more likely that Facebook also has a positive return, and thus $y_{\mathrm{google}, t}$ and $y_{\mathrm{facebook}, t}$ are correlated. It remains open how the correlations between  $y_{\mathrm{google}, t}$ and $y_{\mathrm{facebook}, t}$ may be properly leveraged.  

Keeping in mind the above shortfalls, 
% With the presence of the above weaknesses, 
the following problem remains widely open:
% 
\emph{Is it possible to build an end-to-end machine learning pipeline that leverages  heterogeneous data sources to extract high quality alpha?}


\myparab{Our approach.} We propose a new global framework that integrates different sources of data which may capture different salient/latent structures underlying the same set of financial instruments. Our solution innovates on both the data and methodological sides to circumvent the above limitations in existing models.

\mypara{Data source innovation.} Our solution simultaneously uses multiple categories of signals (heterogeneous data) so that we can extract the ``alphas'' in different ways: (i) Technical signals that are primarily constructed from stocks' prices and their trading volumes~\cite{Fama,stock2011dynamic}, which reflect trading activities in the market, (ii) Financial news signals that indicate the emergence of shocks/events, and (iii) Cross-sectional signals that code the co-movement between similar stocks. 

\mypara{Methodological innovation.} Our framework needs to be computationally and statistically efficient in dealing with heterogeneous signals. Our new methodology possesses three salient properties: (i) \emph{Low overfitting.} 
Although our model uses an extensive collection of technical signals, it generalizes better than linear models. (ii) \emph{Cross-categorical interactions:} our model captures interactions between signals from different categories (e.g., how shocks of one stock and trading volumes of a second stock interact), and (iii) \emph{Low compute cost:} a standard way to extract cross-sectional signals is to use the so-called ``factor model''~\cite{stock2011dynamic}. This often inevitably requires us to run SVD on large datasets. We design a graph-based gadget to extract cross-sectional signal without using SVD. 



\begin{figure*}
\vspace{-2mm}
    \centering
    \includegraphics[scale = 0.3]{figures/framework.pdf}
    \caption{The framework of our end-to-end model. Nodes in the \textsc{Stock2vec} model represent stocks. We learn the stock vector $c_i$ from \textsc{Stock2vec}, factor embedding $g_i^t$ from technical module and news representation $o_i^{t}$ from news module. After that, we feed $[c_i, g_i^t, o_i^t]$ to a sequential model to make prediction on $\hat{y}_i^{t+1}$.}
    \label{fig:framework_new}
\end{figure*}



==> method_old.tex <==
\vspace{1mm}
\section{Our framework}\label{method}
\vspace{1mm}
We consider heterogeneous inputs, the financial news corpus and the stock technical factors, the latter being derived from price and dollar volume in prior trading dates. As shown in Figure.\ref{fig:framework}, the \textsc{Stock2Vec} graph module learns the stock representation. We then integrate the stock embedding with technical factors and news corpus to make the forecast. Next, we will first introduce the design of \textsc{Stock2Vec}.
\subsection{Mining \textsc{Stock2Vec} from news}
\vspace{1mm}

% As motioned before, we aim to obtain effective representations to reflect stock properties based on the rule that stocks with similar properties have similar representations. One straightforward way is to employ human experts to conduct manual labeling. However, this is quite unrealistic as a result of the high requirements of its efficiency and robustness. 
% Instead, we seek to tackle this problem from a data mining view. 

We propose \textsc{Stock2Vec}, which mines the stock embedding from the news because such data comprises a valuable knowledge repository with rich relation information between stocks from the crowd of human intelligence.  Inspired by the observations (Figure~\ref{fig:intro}) that the stocks frequently co-mentioned by the same news are likely to share similar properties and show the co-movements in price.  We formulate the stock co-occurrence matrix and use matrix factorization to extract the static stock representation in Section~\ref{static}. 
To explicitly leverage the cross-sectional signals and circumvent the challenge that the relations between stocks are evolving, we build the temporal stock graph and fine-tune the stock representation by infusing neighbors latent representation dynamically (Section~\ref{dynamic}). 


\subsection{Capture long-term stock relations}\label{static}
\vspace{1mm}
 We now focus on learning the long-term relation and we will discuss how to address the dynamic relations in the next subsection.
\begin{figure}[]
    \centering
    \includegraphics[scale = 0.3]{figures/MF.pdf}
    \vspace{-2mm}
    \caption{Generating the static representations of stocks}
    % \caption{The example of matrix factorization on stock co-occurrence matrix.}
    \label{mf}
    \vspace{-5mm}
\end{figure}

\myparab{Co-occurrence matrix.} 
We build a stock co-occurrence matrix by counting the stock co-occurrence within each news. \qq{why talking about matrix factorization here? }
We prefer matrix factorization on the stock co-occurrence matrix instead of the entire news and stock matrix for the following two reasons: (1) The size of stock co-occurrence matrix only depends on the number of stocks and is much smaller than the news and stock matrix.   (2) We only care about the stock representation, which means the news representations are not necessary. 
We use the global co-occurrence matrix to obtain stable representations that reflect the essential relations between stocks.

%  Co-occurrence~\cite{mikolov2013distributed,pennington2014glove} has proven to be an essential source of information when learning representations of words. 



Formally, assume we have $n$ stocks and $\mX \in \reals^{n\times n}$ is the stock co-occurrence matrix. $\mX_{i, j}$ represents the number of articles that mention both $s_i$ and $s_j$ before testing phase. We associate a vector  $e_i \in \reals^d$ to represent the stock steady representation\qq{steady? static? stable? let's make it consistent. }, where $d$ is the dimension of stock representation.
In this way, the similarity between stock $i$ and stock $j$ can be formulated as the inner product of $e_i$ and $e_j$, which is $e_i^{\transpose}e_j$.

\myparab{Matrix Factorization. } As shown in Figure~\ref{mf}, we adopt a matrix factorization based approach~\cite{koren2009matrix} to learn embedding for the stock node. 
The matrix factorization is one collaborative filtering method. The idea behind matrix factorization is to learn the latent representation where nodes near each other will likely obtain similar embeddings. 
Given the co-occurrence matrix reflect the similarity between stocks, we can get the latent representation of stocks through fitting the training data by optimizing the objective function:
\begin{equation}
\vspace{1mm}
J_s = \sum_{i,j=1}^{n}(e_i^{\transpose} e_j  - \mX_{ij})^2, 
\label{loss_raw}
\vspace{1mm}
\end{equation}

Consider the prior bias of stocks, we introduce the bias items $b_i$ and $b_j$ as the represents the bias of
stock $i$ and stock $j$ to the objective function,

\begin{equation}
J_s = \sum_{i,j=1}^{n}(e_i^{\transpose} e_j  + b_i + b_j - \mX_{ij})^2 + \beta (||\theta||^2)
\label{loss_raw_regu}
\vspace{1mm}
\end{equation}

where the $||\theta|| $ is the learnable parameters including $e_i$, $e_j$, $b_i$ and $b_j$. $\beta (||\theta||^2)$ is the regularization term that prevents overfitting.

%\qq{how to pitch our scheme? We propose two embeddings?  static and dynamic stock embedding? Or we fine-tune the embedding by the propagate }


\subsection{Infuse neighbors' dynamic impact}\label{dynamic}
\vspace{1mm}
The latent representation learned from the above global occurrence matrix reflects the steady and static stock relations. Motivated by the fact that the stock relation is changing over time and cross-asset signals are beneficial towards stock price prediction, we further fine-tune the stock representation by building a temporal stock graph and infusing the neighbors' embedding dynamically.


\myparab{Temporal stock graph}
As shown in Figure~\ref{temporal}, the construction of  $G_t$ consists of two steps.
(1) Construct the stock graph using co-occurrence matrix. Assume $\tilde{G_t} = \{\calv, \cale_t\}$ is the stock graph at time $t$, where $\calv = \{s_1, \dots, s_n\}$ is the set of stocks. $(s_i, s_j) \in \cale_t$ if and only if $s_j$ and  $s_i$ are co-mentioned by the news collected at time $t$. The weight over $s_i$ and $s_j$ is the number of 
co-occurrence from all the news in date $t$.
(2) Due to insufficient number of news about specific stocks in time $t$, we maintain a sliding window $w$ ($w$ is a hyper-parameter) to collect a sequence of stock graphs and then construct $G_t$ by taking a exponential moving average of $\tilde{G}_{t-w+1},...,\tilde{G}_{t-1},\tilde{G}_t$, where we assign the nearby graph a larger weight.
%\qq{mention more details? update the figure subscript}



\myparab{Propagate neighbors' embedding by stock attention mechanism.}
Given the temporal graph ($G_t$) identifies the dynamic stock structure, it is crucial to appropriately update the stock representation by infusing the current neighbors' embedding. 
Motivated by the fact that not all the neighbors contribute to the current stock trend, we filter out the stocks that are too far away from the current stock (See Section~\ref{eff_emd} for more details). Specifically, for stock $s_i$, we focus on the $k$ nearest neighbors that are sorted by the edge weight (the edge weight reflects the magnitude of co-occurrence), where $k$ is a hyper-parameter. Formally, Let $S_t(i)$ be the set of $k$ nearest neighbors of $s_i$ in $G_t$ at time $t$. 

We introduce an attention mechanism~\cite{vaswani2017attention} to infuse the neighbors embedding weighted by an assigned attention value. In this way, we reward the stock offering more forecasting power larger attention value.

\begin{equation} 
    c^i_t = \sum_{j \in S(i)} \alpha_{ij}e_j
    \label{attention}
\end{equation} 
\begin{equation}
    \sum_{j \in S_t(i)} \alpha_{ij} = 1 \textnormal{   for  } j \in S_t(i), 
\vspace{1mm}
\end{equation}
where $c^i_t$ denotes the fine-tuned stock representation for stock $i$ at time $t$, and $\alpha_{i,j} \in \reals$ is the attention weight on the embedding $e_j$, which is given by 
\begin{equation}
\vspace{1mm}
    \alpha_{ij} = \frac{exp(f(e_i,e_j))}{\sum_{l \in S(i)}exp(f(e_i,e_l))}.
    \label{update_alpaha}
    \vspace{1mm}
\end{equation}
The weights define which neighboring stock is more significant. $f(e_i,e_j)$ measures the compatibility between embedding $e_i$ and $e_j$, and is parameterized by a feed-forward network with a single hidden layer, which is jointly trained with other parts of the model. We let $f(\cdot,\cdot)$ have the following functional form:
\begin{equation}
\vspace{1mm}
    f(e_i,e_j) =\mathbf{v}_a^{\transpose} \text{tanh}(\mathbf{W_a}[e_i;e_j] +b_a),
    \vspace{1mm}
\end{equation}
$\mathbf{v}_a$ and $\mathbf{W}_a$ are weight matrices and $b_a$ is the bias vector~\cite{vaswani2017attention} which obtained during model training via backpropagation.


%The attention mechanism can be interpreted as how 



\begin{figure}[]
    \centering
    \includegraphics[scale = 0.35]{figures/temporal_graph.pdf}
    \label{fig:mf}
    \vspace{-3mm}
    \caption{The construction of temporal graph.}\label{temporal}
    \vspace{-4mm}
\end{figure}

\subsection{Sequential modeling}\label{seq} 
\vspace{1mm}


Finally, we integrate the stock embedding from \textsc{Stock2Vec} with stock dynamic features into the neural net model to predict the future return.  The stock dynamic input is $g^i_t$, which comes from technical factors and textual data. We overlay the stock vector $c^i_t$ with $g^i_t$ as an input. Specifically, let $h_t^i$ be the hidden state at time $t$ for stock $i$
\begin{equation}
\vspace{1mm}
    h_t^i = [c^i_t, g^i_t].
    \label{concat_input}
\end{equation}
\vspace{1mm}
where [$\cdot$, $\cdot$] means a direct concatenate.

Considering stocks trend is highly influenced by a variety of time-series market signals, it is intuitive to take the historical status of a stock as the most influential input to predict its future trend. Therefore, we use Recurrent Neural Networks (~\cite{mikolov2010recurrent,schuster1997bidirectional}) as the neural net model. LSTM is a variant of the recurrent net, which is capable of learning long-term dependencies.  The final output is 
\begin{equation}
\vspace{1mm}
    v_{t-T}^i,..., v_{t-1}^i, v_t^i = \text{LSTM}(h_1^i,h_2^i...h_T^i;\theta_l)
    \label{lstm}
    \vspace{1mm}
\end{equation} 
where $\theta_l$ denotes the  parameters from LSTM. 


\myparab{Temporal attention layer.}  Since the stock historical data contributes to the stock trend unequally, we adopt the attention mechanism on the temporal level. We consider 
\begin{equation}
\vspace{1mm}
\begin{matrix}
        r_{t+1}^i = \sum_p \beta_p v_p^i,  \\  \\
\beta_{p} = \frac{exp(f(v_p^i,v_q^i))}{\sum_{q}exp(f(v_p^i,v_q^i))}, 
\end{matrix}
\label{get_r}
\vspace{1mm}
\end{equation}
where $\beta_p$ is the attention weight for prior date $p$ indicating the importance of the date. We then compute the weighted sum to incorporate the sequential data and temporal attention. 

Assume we have $m$ trading days and $n$ stocks. We used the mean squared error as the loss function for gradient descent, given by 
\begin{equation}
J = \frac{1}{mn}\sum_{i=1}^n\sum_{t=1}^{m}(r_{t+1}^i-\hat{r}_{t+1}^i)^{2}.
\label{loss_main}
\vspace{1mm}
\end{equation}
Algorithm~\ref{alg1} describes our entire algorithmic training pipeline.

%\vspace{-4mm}
\qq{I would suggest using two sections for two components... 1) stock embedding 2) heterogeneous sources of input. }

\subsection{Gather difference source of alpha}
\vspace{1mm}

Financial studies have attributed stock movements to three types of market information, i.e., cross-sectional signals, the numerical technical indicators, and the textual media features. In this study, we adopted all three types as described below.

\myparab{Stock graph: leveraging cross-sectional signals.} Trading on cross-sectional signals (i.e., when Google goes up, Facebook is more likely to go up) is remarkably difficult because we need to examine all possible relations. 
%There are approximately $3000 \times 3000 = 1 \mbox{ million}$ interactions, so we face both compute and statistical challenges in controlling the false discoveries rate.
We leverage news articles that mention multiple stocks to detect correlations between stocks' prices. Detecting co-movements by news appears to be much more effective than existing methods.
Our \textsc{Stock2Vec} learns both long-term and evolving relations. 
%We circumvent the problem by building a stock graph, which enables us to identify similar stocks accurately. \qq{udpate}



\myparab{Technical factors: hand-built features are more effective.} We note that features extracted by deep learing~\cite{fengenhancing,rather2015recurrent,doering2017convolutional,lin2017hybrid,ijcai2019-514} are often less effective than features (technical factors) crafted by financial professionals~\cite{colby1988encyclopedia}. Thus, we overlay an LSTM over technical factors so that we can simultaneously use expertise from financial professionals and extract serial correlations from deep learning models.  

\myparab{Textual media}
Advancing development of Natural Language Processing techniques has inspired increasing efforts on stock trend prediction by automatically analyzing stock-related articles~\cite{hu2018listening,chiong2018sentiment,akita2016deep}.
We pre-trained \textsc{Word2vec}~\cite{mikolov2013efficient,mikolov2015computing} on the news corpus from the training data set to produce word embeddings. We average all the word vectors in a piece of news to represent the news vector.  For a given date $t$ and stock $i$, we compute the daily news vector by extracting the news related to stock $i$ and averaging the news vectors within date $t$. 
\lipsum[1-2]
 \begin{algorithm}[t]
\caption{Our model}
\label{alg1}
\begin{algorithmic}[1]
\REQUIRE Online textual corpus, technical factors
\ENSURE Prediction on future $\hat{r}_{t+1}^i$ 
\STATE {Variables: Stock embedding matrix $\mE$, stock attention parameters $\alpha_{i,j}$,  LSTM parameters $\theta_l$, temporal attention parameters $\beta_{i}$.}
\STATE Use the matrix factorization and  loss function (Equation\ref{loss_raw_regu}) to extract stock embedding matrix $\mE$.
\REPEAT
\STATE $s_i$ $\gets$ stock $i$ from universe
\FOR{time stamp $t$}
\STATE Build temporal graph $G_t$
\FOR{stock $j$ in  $S_{i}$} 
    \STATE {Obtain the $\alpha_{i,j}$ with Equation~\ref{update_alpaha}} 
\ENDFOR
\STATE Calculate the stock $i$'s final representation $c^i_t$
\STATE Concatenate with the stock dynamic input to obtain final representation $h_t^i$ with Equation~\ref{concat_input}
%\STATE Get $v_{t-T},..., v_{t-1}, v_t$ by Equation~\ref{lstm}
\STATE Forecast future return $\hat{r}^i_{t+1}$ using Equation~\ref{get_r}.
\ENDFOR
\STATE Calculate prediction loss $J$ by Equation\ref{loss_main}
\STATE Update parameters based on the gradient of $J$  
\UNTIL{convergence}
\label{alg}
\end{algorithmic}
\end{algorithm}

%\myparab{Fundamental data: it only adds noises.} Because our forecasting horizon is only a few days or a week (e.g., the response is the next 5-day return), a company's fundamental data (e.g., its earning, cash flow, book to price ratio, etc.) has only a minimal impact. We find that excluding all the fundamental data will improve our model's generalization error.\qq{remove it if necessary}

\begin{figure*}[t!]
    \centering
    
    \subfigure[Correlation.]{
    \includegraphics[width=0.42\textwidth]{figures/corr.pdf}
    \label{fig:corr}}  \hspace{0.1\textwidth}
    \subfigure[$t$-statistics.]{
    \includegraphics[width=0.42\textwidth]{figures/tstat.pdf}
    \label{fig:tstat} }   % \hspace{0.1\textwidth}
    \caption{Performance comparison for different years in terms of correlation and t-statistic.}
    \label{fig:main_chart}
    \vspace{-2mm}
\end{figure*}

==> new_intro.tex <==
\section{Introduction}
%\qq{add why we need the stock representation}
%\qq{the limitation for existing method using technical factors or return?}

\qq{some questions (1) why use news instead of other source to get the co-occurrence? what's the limitation of other source, such as fundamental and technical features?}

\qq{why we use kNN?}

\qq{the traditional usage of uses and the limitations. use the news sentiments to forecast.}



Forecasting stock prices is a fundamental goal in financial markets.
While there has been extensive research concerning stock prices' predictability, most traditional efforts rely on time series analysis models, such as Autoregressive models CITE, Kalman Filters CITE, technical analysis CITE, etc. 
In general, these solutions use stock prices and volumes to create technical indicators, such as the moving average over dollar volume and volatility over price. They take the historical technical indicators as input to forecast the future stock price trend. {\color{red} The whole paragraph looks non-opt}

However, such traditional solutions yield apparent limitations.
\noindent{\emph{1. Limited capability for distinguishing the future profits of different stocks. }}
As the technical analysis {\color{red} indicator not defined, technical analysis not elaborated} does not distinguish the difference between stocks {\color{red} some earlier works addressed this issue?}, the 
a unified transformation {\color{red} what is unified transformation, as opposed to what} over price and volume for all the stocks has 
certain limitations for the task of selecting stocks with higher future profits {\color{red} this sentence does not parse either}.
Stocks with different natures have different affinities over indicators.
For example, the high price volatility is a valuable indicator for a steady and mature stock. 
However, for the cyclical stocks whose price rises and falls with the business cycle, the extreme price volatility is routine and has few effects to reference. {\color{red} prior works did that?}

\noindent{\emph{2. Cross-sectional effects are not properly leveraged.}} {\color{red} our model is not a cross asset model?}
The existing methods typically treat stocks as independent of each other and ignore the relations between stocks. However, a salient property of the equity return forecasting problem is that the training pairs $(X, y)$ are not independent. For example, when Google has a positive return, it is more likely that Facebook also has a positive return, and thus $y_{\mathrm{google}, t}$ and $y_{\mathrm{facebook}, t}$ are correlated. 
It remains open how the correlations between  $y_{\mathrm{google}, t}$ and $y_{\mathrm{facebook}, t}$ may be properly leveraged. {\color{red} this paper did not address this issue? I think we still have not highlight this paper's major contribution and how we differ from existing one. } 


\begin{figure}[t!]
    \centering
    \subfigure[The frequent co-mention captures sector relation between stocks]{
    \includegraphics[scale = 0.20]{figures/intro1_news.pdf}\label{fig:sec}
    }
    \subfigure[The frequent co-mention captures supply chain relation between stocks]{
    \includegraphics[scale = 0.195]{figures/intro2_news.pdf}\label{fig:supply}}
    \caption{Two examples of stock time series data in terms of price increasing rate from two pairs of frequent co-mentioned stocks and the examples for corresponding
    news.}
    \vspace{-10 pt}
    \label{fig:intro}
\end{figure}



To address these limitations,  
we believe it is quite beneficial to take into account each stock’s latent representation. CITE 
The stock representation naturally reflects stocks' nature (e.g., distinguish the steady stocks from the cyclical) and captures dynamic interactions between signals from different categories (e.g., how shocks from one stock's price and trading volume impact the others). {\color{red} we did not do it.}
In this paper, we propose Stock2Vec and integrate Stock2Vec into the existing deep neural networks approach with widely-used dynamic stock indicators.   
%we propose integrating the stock’s latent representation (Stock2Vec) into the existing deep neural networks approach with widely-used dynamic stock indicators.   
To realize this idea, however, it is requisite to answer two challenging research questions: 1) how to extract and represent the stock latent representation? {\color{red} CHECK usage of ``how to''}  2) how to integrate the stock latent representation into the existing deep neural networks approach to enhance the dynamic stock prediction?

The effective representation should be able to distinguish stocks from each other, reflect the similarity between stocks {\color{red} this is a non-opt; what latent representation does not reflect similarity?}. Intuitively, it is more practical and effective to build a stock representation based on diverse aspects of human experts' intuition and knowledge{\color{red} make sure the rest of the paper connects back to this point. feels you are heading towards doing some HCI?}.  One straightforward way is to collect such information manually from experts and analysts. However, it is low efficiency and costly. 
Fortunately, millions of investors, analysts, and financial experts share opinions, events, transactions in real-time{\color{red} this pitch sounds very 20 years ago; i think we can just articulate what technical problems need to be solved.}. Online media content is indeed a gold mine in reflecting market trends and volatility since it covers intelligence and knowledge {\color{red} non-opt.}. 

\qq{Due to the highly abstract and summary nature of news,}  numerous news contains more than one stock entity {\color{red} your discussion suddenly move from very high-level ``gold mine'' to very low level; try to articulate where you are heading.}. Through the statistic analysis of real-world online stock news (collected from Sina), a piece of news refers to 2.94 stocks on average. 
Notably, we find that when two stocks are frequently co-mentioned, they tend to yield a similar stock trend. For instance,  Fig.~\ref{fig:intro} illustrates the time series for price increasing rate from two pairs of frequently co-mentioned stocks. We can observe that the fluctuations of two curves in Fig.~\ref{fig:sec} and Fig~\ref{fig:supply} are great synchronous.  It is a clear indication that the news co-mention reveals the stock intrinsic relation such as sector relation and supply chain relation. Based on this observation, we assume that stocks within the same news are likely to share some common characteristics. Therefore, we use the news co-mention to learn the stock representation. We formulate the stock co-occurrence matrix from news and initial the stock representation using matrix factorization {\color{red} it seems this paragraph contains the entire contribution and sounds ``thin''. Also need to connect back to the major limitation you mentioned earlier. Also, the regularization is not mentioned?}



%build the stock graph based on the co-occurrence between stocks in ne.\qq{use news to build the stock graph}
\begin{figure}[t]
    \centering
    \includegraphics[scale = 0.28]{figures/stock2vecd.pdf}
    \caption{The illustration of Stock2Vec. Each solid circle represents a stock. The final representation of a stock is computed by smoothing its neighbors' basic embedding via the attention mechanism. After that, we use the stock embedding and its dynamic inputs to represent the current stock status, which is then fed to a neural network model to make the final prediction.}
    \label{fig:dyanmaic}
\end{figure}

%
\qq{The impact of noises canceled out by neighbors; leverage neighbor information;Computational efficiency; the impact of neighbors are evolving}

After obtaining the representations of stock intrinsic properties, the next question remains how to integrate the stock embedding into the existing deep neural networks approach. A straightforward way is to directly append stock properties' representations with the dynamic stock indicator as the unified input into the deep neural networks. However, this method ignores the fact that the relation between stocks is evolving. We design the graph-based component use near-neighbor based approach to learn the stock representations dynamically. The process of resorting to the neighbors can be automated via the attention mechanism and the end-to-end training described in Fig~\ref{fig:dyanmaic}.




To validate the effectiveness of Stock2Vec, we perform extensive experiments on real-world data that contains more than 3000 stocks in the Chinese stock market from 2012 to 2018. The experiment results demonstrate the effectiveness of stock representation extracted from news co-mentions in stock prediction. The further market trading simulation illustrates that our proposed approach can result in a significant increment of profit. To sum up, our contributions are three-fold:

\begin{itemize}
    \item We remark that our way to use news data sets deviates from standard news-based models for predicting equity returns~\cite{ding2015deep,hu2018listening}. Most news-based models aim to extract sentiments and events that could directly impact one or more related stocks' prices. To our best knowledge, this work is among the first to mine the representation for stocks from the news co-mention.   
    \item Develop the neighbor-based smoothing method as regularization to fine-tune the stock evolving representation.
    \item 
     We perform extensive experiments on data sets on real-world market to confirm the efficacy of extracted stock representation for stock trend prediction.
\end{itemize}
\iffalse
content from online media has indeed become a gold mine for investors to understand market trends and volatility.


To pursue more accurate stock prediction, it is quite beneficial to take into account each stock’s intrinsic properties. 

In this paper, we propose to integrate the stock’s intrinsic properties into the existing deep neural networks approach. To this definitive end, however, it is requisite to answer two challenging questions: 1) how to extract and represent the stock intrinsic properties? 2) how to integrate the static intrinsic properties into the existing deep neural networks approach to enhance the dynamic stock prediction.

Online forums and stock investment websites such as Stock- twits, Twitter and Weibo allow millions of investors to share transactions, opinions, news events and so on in real time. The numerous public comments are of great value in reflect- ing market conditions and making trading decisions, which have been well studied in recent years. 


Due to the highly abstract nature of stock intrinsic properties. There is hardly a comprehensive and clear definition of such intrinsic properties in human investors’ minds. Moreover, such intrinsic properties could cover a couple of diverse aspects of human investors’ intuition and knowledge. Therefore, investment behaviors of human investors could be an indispensable information to recognize such intrinsic properties. Fortunately, mutual fund portfolio data, consisting of investment behaviors of expert investors, forms a gold mine for mining stock intrinsic properties.
\fi


